Localized Dimension Growth: A Convolutional Random Network Coding Approach to Managing Memory and Decoding Delay

We consider an \textit{Adaptive Random Convolutional Network Coding} (ARCNC) algorithm to address the issue of field size in random network coding for multicast, and study its memory and decoding delay performances through both analysis and numerical simulations. ARCNC operates as a convolutional code, with the coefficients of local encoding kernels chosen randomly over a small finite field. The cardinality of local encoding kernels increases with time until the global encoding kernel matrices at related sink nodes have full rank.ARCNC adapts to unknown network topologies without prior knowledge, by locally incrementing the dimensionality of the convolutional code. Because convolutional codes of different constraint lengths can coexist in different portions of the network, reductions in decoding delay and memory overheads can be achieved. We show that this method performs no worse than random linear network codes in terms of decodability, and can provide significant gains in terms of average decoding delay or memory in combination, shuttle and random geometric networks.

==> algorithm.tex <==
\subsection{Success probability}

Discussions in \cite{HMK2006, LYC2003, KM2003} state that in a
network with delays, ANC gives rise to random processes which can be
written algebraically in terms of a delay variable $z$. In other
words, a convolutional code can naturally evolve from the message
propagation and the linear encoding process. ANC in the delay-free
case is therefore equivalent to CNC with constraint length 1.
Similarly, using a CNC with constraint length $l>1$ on a delay-free
network is equivalent to performing ANC on the same network, but
with $l-1$ self-loops attached to each encoding node. Each self-loop
carries $z, z^2, \ldots, z^{l-1}$ units of delay respectively.

For example, in Figure~\ref{fig:ANC_CNC}, we show a node with two incoming edges.  Let the data symbol transmitted on edge $\dot{e}$ at time $t$ be $y_{\dot{e},t}$. A CNC with length $l=2$ is used on the left, assuming that transmissions are delay free. According to Eq.~\eqref{eq:yet_k} and \eqref{eq:yet}, the data symbol transmitted on $e_1$ at time $t$ is
\begin{align}
y_{e_1,t} & = \sum_{\dot{e}\in\{e',e''\}} y_{\dot{e},t}k_{\dot{e},e,0}+y_{\dot{e},t-1}k_{\dot{e},e,1}\,. \label{ye1tCNC}
\end{align}
%
On the right, the equivalent ANC is shown for the same node, where a single loop with a transmission delay of 1 has been added. Using a matrix notation, the output data symbols from $v$ are $(y_{e_2,t} \quad y_{e''',t}) = (y_{e',t} \quad y_{e'',t} \quad y_{e''',t-1})K_v $, i.e.,
\begin{align}
% (y_{e_2,t} \quad y_{e''',t}) & = (y_{e',t} \quad y_{e'',t} \quad y_{e''',t-1})K_v \\[4pt]
%\text{i.e.} \quad \quad y_{e''',t} & = y_{e',t}k_{e',e,1} +y_{e'',t}k_{e'',e,1}\notag \\
    y_{e''',t} & = y_{e',t}k_{e',e,1} +y_{e'',t}k_{e'',e,1}\notag \\
    y_{e_2,t}& = y_{e',t}k_{e',e,0}+y_{e'',t}k_{e'',e,0}+y_{e''',t-1} \notag \\
    & = \sum_{\dot{e}\in\{e',e''\}} y_{\dot{e},t}k_{\dot{e},e,0}+y_{\dot{e},t-1}k_{\dot{e},e,1} \label{ye2tANC}
\end{align}

\begin{figure}[t!]
  \centering
  \includegraphics[width=3.4in]{./graphics/ANC_CNC.eps}\\
  \caption{A convolution code resulting from self-loops on a network with transmission delays. (a) CNC in a delay-free network. Data transmitted on incoming edges are $y_{e'}(z)$ and $y_{e}(z)$ respectively. The local encoding kernels are given by $K_{\text{CNC}}(z)$. (b) Equivalent ANC in a network with delays. The given self-loop carries a single delay $z$. Data symbols transmitted on incoming edges are $y_{e',t}$ and $y_{e'',t}$ at time $t$. The ANC coding coefficients are given by the matrix $K_{\text{ANC}}$.}\label{fig:ANC_CNC}
\end{figure}

Clearly $y_{e_1,t}$ is equal to $y_{e_2,t}$. The ARCNC algorithm we have proposed therefore falls into the framework given by Ho et al. \cite{HMK2006}, in the sense that the convolution process either arises naturally from cycles with delays, or can be considered as computed over self-loops appended to acyclic networks. Applying the analysis from \cite{HMK2006}, we have the following theorem,

\begin{theorem}\label{thm:prob}
For multicast over a general network with $d$ sinks, the ARCNC algorithm over $\mathbb{F}_q$
can achieve a success probability of at least $(1-d/q^{t+1})^{\eta}$ at time $t$, if $q^{t+1}>d$, and $\eta$ is the number of links with
random coefficients.
\end{theorem}

\begin{proof} At node $v$, the local encoding kernel $k_{e',e}(z)$ at time $t$ is a polynomial with maximal degree $t$, i.e.,  $k_{e',e}(z)=k_{e',e,0}+k_{e',e,1}z+\cdots+k_{e',e,t}z^{t}$, where $k_{e',e,i}$ is randomly chosen over $\mathbb{F}_q$. If we group the encoding coefficients, the ensuing vector, $k_{e',e}=\{k_{e',e,0},k_{e',e,1},\cdots,k_{e',e,t}\}$, is of
length $t+1$, and corresponds to a random element over the extension field
 $\mathbb{F}_{q^{t+1}}$. Using the result in \cite{HMK2006}, we conclude that the success probability of ARCNC at time $t$ is at least $(1-d/q^{t+1})^{\eta}$, as long as $q^{t+1}>d$.
\end{proof}

We could similarly consider the analysis done by Balli et al. \cite{BYZ2009}, which states that the success probability is at least
$(1-d/(q-1))^{|J|+1}$, $|J|$ being the number of encoding nodes, to show that a tighter lower bound can be given on the success probability
of ARCNC, when $q^{t+1}>d$.

\subsection{First decoding time}\label{sec:stoppingTime}
As discussed in Section~\ref{subsubsec:decoding}, we define the \emph{first decoding time} $T_r$ for sink $r$, $1\leq r\leq d$, as the time it takes $r$ to achieve decodability for the first time. We had called this variable the \emph{stopping time} in our previous work \cite{guo2011localized}. Also recall that when all sinks are able to decode, at each individual sink $r$, $T_r$ can be smaller than $L_r$, which is the degree of the global encoding kernel matrix $F_r(z)$. Denote by $T_N$ the time it takes for all sinks in the network to successfully decode, i.e., $T_N=\max\{T_1,\ldots,T_d\}$, then $T_N$ is also equal to $\max\{L_1,\ldots,L_d\}$. The following corollary holds:

\begin{corollary}
For any given $0<\varepsilon<1$, there exists a $T_0>0$ such that for any $t \geq T_0$, ARCNC solves the multicast problem with probability
at least $1-\varepsilon$, i.e., $P(T_N > t)  < \varepsilon$.\label{crlry2}
\end{corollary}
\proof Let $T_0  = \left\lceil \log_q d-\log_q(1-\sqrt[\eta]{1-\epsilon}) \right\rceil -1 $, then $T_0 + 1 \geq \lceil \log_q d \rceil$ since
$0 < \varepsilon <1$, and $(1-d/q^{T_0+1})^\eta>1-\varepsilon$. Applying Theorem~\ref{thm:prob} gives $P(T_N > t) \leq P(T_N >T_0) <
1-(1-d/q^{t+1})^{\eta}< \varepsilon$ for any $t\geq T_0$,
\endproof
Corollary~\ref{crlry2} shows that $T_N$ is a valid random variable, and ARCNC converges in a finite amount of time for a multicast connection.

Another relevant measure of the performance of ARCNC is the \emph{average first decoding time}, $T_{\text{avg}}=\frac{1}{d}\sum_{r=1}^{d}T_r$. Observe that $E[T_{\text{avg}}] \leq E[T_N]$, where
\begin{align*}
  E[T_N] %& =\sum_{t=0}^{\infty}tP(T_N=t)\\
   & = \sum_{t=1}^{\lceil \log_q d\rceil -1}P(T_N\geq t) + \sum_{t= \lceil \log_q d\rceil}^{\infty}{P(T_N\geq t)}\\
         & \le \lceil \log_q d\rceil -1 + \sum_{t=\lceil \log_q d\rceil}^{\infty}[1-(1-\frac{d}{q^t})^{\eta}] \\
         & = \lceil \log_q d\rceil -1 + \sum_{k=1}^{\eta}(-1)^{k-1}{\eta \choose                                                         k} \frac{d^k}{q^{\lceil \log_q d\rceil k}-1}\,.
\end{align*}
%
When $q$ is large, the summation term becomes $1-(1-d/q)^\eta$ by the binomial expansion.  Hence as $q$ increases, the second term above diminishes to $0$, while the first term $\lceil \log_q d\rceil -1$ is 0. $E[T_{\text{avg}}]$ is therefore upper-bounded by a term converging to 0; it is
also lower bounded by 0 because at least one round of random coding is required. Therefore, $E[T_{\text{avg}}]$ converges to $0$ as $q$ increases.  In other words, if the field size is large enough, ARCNC reduces in effect to RLNC.

Intuitively, the average first decoding time of ARCNC depends on the network topology. In RLNC, all nodes are required in code in finite fields of the same size; thus the effective field size of RLNC is determined by the worst case sink. This scenario corresponds to having all nodes stop at $T_N$ in ARCNC. ARCNC enables each node to decide locally what is a good constraint length to use, depending on side information from downstream nodes. Since $E[T_{\text{avg}}]\leq E[T_N]$, some nodes may be able to decode before $T_N$. The corresponding effective field size is therefore expected to be smaller than in RLNC. Two
possible consequences of a smaller effective field size are reduced decoding delay, and reduced memory requirements. In Section~\ref{sec:examples}, we confirm through simulations that such gains can be attained by ARCNC.

\subsection{Memory}\label{sec:memory}

To measure the amount of memory required for ARCNC, first recall from Section~\ref{sec:basicDefs} that at each node $v$, the global encoding kernel matrix $F_v(z)$, the local encoding kernel matrix $K_v(z)$, and past data $y_{e'}(z)$ on incoming arcs $e'\in In(v)$ need to be stored in memory. $K_v(z)$ and $y_{e'}(z)$ should always be saved because together they generate new data symbols to transmit (see Eq.~\eqref{eq:yet_k} and \eqref{eq:yet}). $F_v(z)$ should be saved during the code construction process at intermediate nodes, and always at sink nodes, since they are needed for decoding.

Let us consider the three contributors to memory use one by one. Firstly, recall from Section~\ref{sec:basicDefs} that $F_v(z)$ can be viewed as a polynomial in $z$. When all sinks are able to decode, at an individual node $v$, $F_v(z)$ has degree $L_v$, and coefficients from $\mathbb{F}_q^{m\times In(v)}$. The total amount of memory needed for $F_v(z)$ is therefore proportional to $\lceil\log_2 q\rceil m In(v) (L_v+1)$. Secondly, from Eq.~\eqref{eq:fet}, we see that the length of a local encoding kernel polynomial $k_{e',e}(z)$ should be equal to or smaller than that of $f_e(z)$. Thus, the length of $K_v(z)$ should also be equal to or smaller than that of $F_v(z)$. The coefficients of $K_v(z)$ are elements of $\mathbb{F}_q^{In(v)\times Out(v)}$. Hence, the amount of memory needed for $K_v(z)$ is proportional to $\lceil\log_2 q\rceil Out(v) In(v) (L_v+1)$. Lastly, a direct comparison between Eq.~\eqref{eq:yet} and \eqref{eq:fet} shows that memory needed for $y_{e'}(z)$, $e'\in In(v)$ is the same for memory needed for $F_v(z)$. In practical uses of network coding, data can be transmitted in packets, where symbols are concatenated and operated upon in parallel. Packets can be very long in length. Nonetheless, the exact size of data packets is irrelevant for comparing memory use between different network codes, since its effect cancels out during comparisons.

Observe that, $m$ is the number of symbols in the source message, determined by the min-cut of the multicast connection, independent of the network code used. Similarly, $In(v)$ and $Out(v)$ are attributes inherent to the network topology. To compare the memory use of different network codes, we can omit these terms, and define the average memory use of ARCNC by the following common factor:
\begin{align}
W_{\text{avg}} \triangleq \frac{\lceil\log_2 q\rceil}{|\mathcal{V}|}\sum_{v\in\mathcal{V}}(L_v+1)\,.\label{eq:Wavg}
\end{align}
\noindent In RLNC, $L_v=0$, and the expression simplifies to $\lceil\log_2 q\rceil$, which is the amount of memory needed for a single finite field element. In Section~\ref{example:umbrella}, we examine the memory overheads of ARCNC in a family of networks called umbrella networks by considering $E[W_\text{avg}]$. In Section~\ref{sec:simulations}, we plot $E[W_{\text{avg}}]$ for several structured and random networks.

\subsection{Complexity}
to study the computation complexity of ARCNC, first observe that, once the adaptation process terminates, the computation needed for the ensuing code is no more than a regular CNC. In fact, the expected computation complexity is proportional to the average code
length of ARCNC. We therefore omit the details of the complexity analysis of regular CNC here and refer interested readers to \cite{EF2004}.

For the adaptation process, the encoding operations are described by Eq.~\eqref{eq:fet}. If the algorithm stops at time $T_N$, then the number of operations in the encoding steps is $O(D_{in}|\mathcal{E}|T_N^2m)$, where $D_{in}$ represents the maximum input degree over all nodes, i.e., $D_{in}=\max_{v\in\mathcal{V}}|In(v)|$.

To determine decodability at a sink $r$, we check if the rank of the global encoding matrix $F_r(z)$ is $m$. A straight-forward approach is to check whether the determinant of $F_r(z)$ is a non-zero polynomial. Alternatively, Gaussian elimination could also be applied. At time $t$, because $F_r(z)$ is an $m \times |In(r)|$ matrix and each entry is a polynomial with degree $t$, the complexity of checking whether $F_r(z)$ is full rank is $O(D_{in}^22^mmt^2)$. Instead of computing the determinant or using Gaussian elimination directly, we propose to check the conditions given in Section~\ref{sec:algAcyclic}. For each sink $r$, at time $t$, determining $rank\left({\begin{array}{*{20}c} F_0 & F_1 & \cdots F_{t} \end{array}}\right)$ requires a computation complexity of $O(D_{in}^2mt^2)$. If the first test passes, we then need to calculate $rank(M_{t})$ and $rank(M_{t-1})$. Observe that $rank(M_{t-1})$ was computed during the last iteration. $M_t$ is a $(t+1)m \times (t+1)|In(r)|$ matrix over field $\mathbb{F}_q$. The complexity of calculating $rank(M_t)$ by Gaussian elimination is $O(D_{in}^2mt^3)$. The process of checking decodability is performed during the adaptation process only, hence the computation complexity here can be amortized over time after the coding coefficients are determined. In addition, as decoding occurs symbol-by-symbol, the adaptation process itself does not impose any additional delays.


==> simu_umbrella.tex <==
\subsection{Umbrella Network}\label{subsec:simuUmbrella}

\begin{figure}[t!]
  \centering
  \includegraphics[width=8.5cm]{./graphics/umbrella_alpha5_beta3to10_qq2.eps}\\
  \caption{Average first decoding time and average memory use in an umbrella network. $\alpha=5$, $\beta$ is between 3 to 10, field size is $q=2^2$.}
  \label{fig:umbrella_alpha5_beta3to10}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=8.5cm]{./graphics/umbrella_beta3_alpha5to30_qq2.eps}\\
  \caption{Average first decoding time and average memory use in an umbrella network. $\beta=3$, $\alpha$ is between 5 and 29, field size is $q=2^2$.}
  \label{fig:umbrella_beta3_alpha5to30}
\end{figure}

Figures~\ref{fig:umbrella_alpha5_beta3to10} and \ref{fig:umbrella_beta3_alpha5to30} plot the average first decoding time and average memory use in umbrella networks when $q=2^2$. Figure~\ref{fig:umbrella_alpha5_beta3to10} shows the performance of ARCNC when the number of layer in the umbrella is increased from $\beta=3$ to 10, while the number of nodes in the top Layer 1, is kept constant at $2\alpha= 10$. With each additional level, two more nodes are added to the set of sinks, and the maximum depth of sinks is incremented by 1. The resulting $T_{\text{avg}}$ and $W_{\text{avg}}$ are approximately linear in $\beta$, increasing in value as $\beta$ becomes larger. When $\beta=10$, $T_{\text{avg}}$ is approximately 2.0, and $W_{\text{avg}}$ is approximately 11.9. Since $\alpha=5$, the number of sinks in the network is $\alpha+2\beta=25$, and the number of coding nodes is $10$, including the source. Similar to the combination network case discussed in the previous subsection, to achieve a decoding probability of 0.99, we have $(1-25/(q-1))^{10+1}\geq0.99$, thus $q>2.7\times10^4$, and $W_{avg,\text{RLNC}}=\lceil \log_2q \rceil \geq 15$, slightly larger than $W_{avg,\text{ARCNC}}$.

Figure~\ref{fig:umbrella_beta3_alpha5to30} shows the performance of ARCNC when there are only $\beta=3$ layer in the umbrella, while $\alpha$ increases from 5 to 29. Unlike in Figures~\ref{fig:umbrella_alpha5_beta3to10}, both $T_{\text{avg}}$ and $W_{\text{avg}}$ decreases as $\alpha$ becomes larger. This is because, first, the added sinks in Layer 1 do not affect code generation for nodes on the handle of the umbrella; second, unlike the combination network, each sink in Layer 1 shares parents with only two other sinks in Layer 1. When $\alpha=29$, $W_{\text{avg}}$ is approximately 4. We can also compute in this case $W_{avg,\text{RLNC}}=\lceil \log_2q \rceil \geq 14$, 2.5 times more than $W_{avg,\text{ARCNC}}$. When $\alpha$ becomes even larger, the gain in  memory use can be even larger when ARCNC is used instead of RLNC. 

==> simulations.tex <==
We have shown analytically that ARCNC converges in finite steps with probability 1, and that it can achieve significant gains in decoding delay or memory, depending on the network under study. In what follows, we want to verify these results through simulations, and study numerically whether similar behaviors can be observed in other structured and random networks.

\subsection{Combination Network}\label{subsec:simuCombination}
\subsubsection{fixed m} In Section~\ref{example:combination}, we computed upper and lower bounds for the expected decoding delay on combination networks. We have also simulated the ARCNC encoder and decoder in Matlab. Figure~\ref{fig:combination_fixedM_2_n} plots these upper bounds, as well as an upper bound for the standard deviation of $E[T]$. Observe that the average decoding delay is only slightly more than 1, even though there are more receivers in the network. The estimated upper and lower bounds for the average decoding delay are independent of the value of $n$.
%
\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/combination_fixedM_2_n.eps}\\
  \caption{Computed upper and lower bounds on the expected decoding delay for combination networks. $m$ is fixed the value of 2, while $n$ increase in value. Field size $q=2$.}
  \label{fig:combination_fixedM_2_n}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/combination_fixedM_2_qq.eps}\\
  \caption{$m$ is fixed the value of 2, while $n$ increase in value. Field size varies.}
  \label{fig:combination_fixedM_2_qq}
\end{figure}

\subsubsection{m proportional to n}
In the case where $m$ is comparable to the number of $n$, we simulate the behavior of the system when $n$ is increased. Figure~\ref{fig:combination_variedM_nOver2} illustrates the estimated upper and lower bounds for the average decoding delay when $m$ and $n$ are comparable in magnitude. Here we have set $m=n/2$. Comparing the simulation results with Figure~\ref{fig:combination_fixedM_2}, we see that a larger decrease in average decoding delay can be observed, even though the number of sinks in the network has increased significantly. For example, when $n=12$, $m=6$, there are 924 sinks for which transmission demands need to be satisfied, compared with 66 sinks when $n=12$ and $m=2$. The upper and lower bound we have computed depends on $n$ since $m$ is linear in $n$.

%\begin{figure}[t!]
%  \centering
%  \includegraphics[width=7.5cm]{./graphics/combination_variedM_nOver2.eps}\\
%  \caption{Computed upper and lower bounds on the expected decoding delay for combination networks. $m$ is set to $n/2$, while $n$ increase in value.}
%  \label{fig:combination_variedM_nOver2}
%\end{figure}

In combination networks, simulation results have verified that decodability can be achieved with probability 1.

\subsection{Umbrella Network}\label{subsec:simuUmbrella}

Figures~\ref{fig:umbrella_alpha5_beta3to10} and ~\ref{fig:umbrella_beta3_alpha5to30} plot the probability of successful decoding, average decoding delay, and average code length in umbrella networks. Figure~\ref{fig:umbrella_alpha5_beta3to10} compares the performance of ARCNC when $\beta$, the number of levels in the network, is set to 3, while the number of nodes in the top layer, $2\alpha$, is kept constant. Since there are more sinks in the network, and the maximum depth of sinks increases with $\beta$, the average decoding delay and average code length also increase linearly in $\beta$. On the other hand, when $\beta$ is kept constant at 3, while $\alpha$ increases, the average decoding delay and average code lengths decrease, since the added sinks does not affect the code generation for nodes on the handle of the umbrella.

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/umbrella_alpha5_beta3to10_qq2.eps}\\
  \caption{Average decoding delay and average code length. $\alpha=5$, $\beta$ is between 3 to 10, field size is $2^2$.}
  \label{fig:umbrella_alpha5_beta3to10}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/umbrella_beta3_alpha5to30_qq2.eps}\\
  \caption{Average decoding delay and average code length. $\beta=3$, $\alpha$ is between 5 and 30, field size is 4.}
  \label{fig:umbrella_beta3_alpha5to30}
\end{figure}

\subsection{Acyclic Random Geometric Networks}\label{subsec:simuAcyclicRandom}
To see the performance of ARCNC in acyclic random networks, we use random geometric graphs \cite{newman2003random} as the network model, with added acyclic constraints. In random geometric graphs, nodes are put into a geometrically confined area $[0,1]^2$, with the coordinates chosen uniformly randomly. Nodes which are within a given distance $d$ are connected. The graph is inherently undirected. In our simulations, we number all of the nodes in the network, with the source as node 1, and the sinks as the nodes with the largest numbers. We assume that a node can transmit to only nodes with number higher than its own. Sinks are also chosen uniformly randomly from all of the non-source nodes. An intermediate node on a path from the source to a sink can be a sink itself. To ensure the max-flow to each receiver is non-zero, one can choose the value of $d$ to make the graph connected with high probability. In our simulations, we throw away instances where any receiver is not connected to the source. Once a acyclic random geometric network is generated, we find the min-cuts of each of the sink nodes, and use the smallest min-cut over all sinks as the number of symbols that the source is sending out at each time instant

Figures~\ref{fig:random_acyclic_total25_rx2to6_qq2_sinksLast} and \ref{fig:random_acyclic_total10to45_rx3_qq2_sinksLast} plot the average decoding delay and average code length in acyclic random geometric networks, when the radius of connection is set to $0.4$. A sink can be on the path from the source to another sink.

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/random_acyclic_total25_rx2to6_qq2_sinksLast.eps}\\
  \caption{Average decoding delay and average code length for a acyclic random geometric graph with 25 nodes, as a function of the number of receivers, field size is 4.}
  \label{fig:random_acyclic_total25_rx2to6_qq2_sinksLast}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/random_acyclic_total10to45_rx3_qq2_sinksLast.eps}\\
  \caption{Average decoding delay and average code length for a acyclic random geometric graph with 3 receivers, as a function of the total number of nodes in the network, field size is 4.}
  \label{fig:random_acyclic_total10to45_rx3_qq2_sinksLast}
\end{figure}

\subsection{Shuttle Network}\label{subsec:simuShuttle}
When there are cycles in the network, we randomly remove edges from lower numbered nodes to the higher numbered nodes one by one until the network becomes acyclic.

Figure~\ref{fig:shuttle_qq} plots the average decoding delay and average code length for the shuttle network.

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/shuttle_qq.eps}\\
  \caption{Average decoding delay and average code length for the shuttle network as a function of field size.}
  \label{fig:shuttle_qq}
\end{figure}
\subsection{cyclic random networks}\label{subsec:simuCyclicRandom}

Cyclic networks are of strong importance to our study, as the

Figures~\ref{fig:random_cyclic_total25_rx2to6_qq2_sinksLast} and \ref{fig:random_cyclic_total10to45_rx3_qq2_sinksLast} plot the average decoding delay and average code length in cyclic random geometric networks, when the radius of connection is set to $0.4$.

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/random_cyclic_total25_rx2to6_qq2_sinksLast.eps}\\
  \caption{Average decoding delay and average code length for a cyclic random geometric graph with 25 nodes, as a function of the number of receivers, field size is 4.}
  \label{fig:random_cyclic_total25_rx2to6_qq2_sinksLast}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=7.5cm]{./graphics/random_cyclic_total10to45_rx3_qq2_sinksLast.eps}\\
  \caption{Average decoding delay and average code length for a cyclic random geometric graph with 3 receivers, as a function of the total number of nodes in the network, field size is 4.}
  \label{fig:random_cyclic_total10to45_rx3_qq2_sinksLast}
\end{figure}
